The permuto-associahedron revisited

A classic problem connecting algebraic and geometric combinatorics is the realization problem: given a poset, determine whether there exists a polytope whose face lattice is the poset. In 1990s, Kapranov defined a poset as a hybrid between the face poset of a permutohedron and that of an associahedron, and he asked whether this poset is realizable. Shortly after his question was posed, Reiner and Ziegler provided a realization. Based on our previous work on the nested braid fan, we provide in this paper a different realization of Kapranov's poset by constructing the vertex set and the normal fan of a permuto-associahedron simultaneously.

==> tikz/loday3.tex <==
\begin{tikzpicture}%
	[x={(0.178656cm, 0.726606cm)},
	y={(-0.806737cm, 0.494173cm)},
	z={(0.563256cm, 0.477323cm)},
	scale=2.00000,
	back/.style={loosely dotted, thin},
	edge/.style={color=black, thick},
	facet/.style={fill=yellow,fill opacity=0.400000},
	vertex/.style={inner sep=1pt,circle,draw=green!25!black,fill=green!75!black,thick,anchor=base}]
%
%
%% Coordinate of the vertices:
%%
\coordinate (-3.00000, -2.00000, 2.00000) at (-3.00000, -2.00000, 2.00000);
\coordinate (-3.00000, 2.00000, -2.00000) at (-3.00000, 2.00000, -2.00000);
\coordinate (-2.00000, -3.00000, 2.00000) at (-2.00000, -3.00000, 2.00000);
\coordinate (-2.00000, 3.00000, -2.00000) at (-2.00000, 3.00000, -2.00000);
\coordinate (0.00000, -3.00000, 0.00000) at (0.00000, -3.00000, 0.00000);
\coordinate (0.00000, -1.00000, -2.00000) at (0.00000, -1.00000, -2.00000);
\coordinate (0.00000, 1.00000, 2.00000) at (0.00000, 1.00000, 2.00000);
\coordinate (0.00000, 3.00000, 0.00000) at (0.00000, 3.00000, 0.00000);
\coordinate (1.00000, 0.00000, -2.00000) at (1.00000, 0.00000, -2.00000);
\coordinate (1.00000, 0.00000, 2.00000) at (1.00000, 0.00000, 2.00000);
\coordinate (2.00000, -1.00000, 0.00000) at (2.00000, -1.00000, 0.00000);
\coordinate (2.00000, 0.00000, -1.00000) at (2.00000, 0.00000, -1.00000);
\coordinate (2.00000, 0.00000, 1.00000) at (2.00000, 0.00000, 1.00000);
\coordinate (2.00000, 1.00000, 0.00000) at (2.00000, 1.00000, 0.00000);
%%
%%
%% Drawing edges in the back
%%
\draw[edge,back] (-3.00000, 2.00000, -2.00000) -- (0.00000, -1.00000, -2.00000);
\draw[edge,back] (-2.00000, -3.00000, 2.00000) -- (0.00000, -3.00000, 0.00000);
\draw[edge,back] (-2.00000, 3.00000, -2.00000) -- (1.00000, 0.00000, -2.00000);
\draw[edge,back] (0.00000, -3.00000, 0.00000) -- (0.00000, -1.00000, -2.00000);
\draw[edge,back] (0.00000, -3.00000, 0.00000) -- (2.00000, -1.00000, 0.00000);
\draw[edge,back] (0.00000, -1.00000, -2.00000) -- (1.00000, 0.00000, -2.00000);
\draw[edge,back] (1.00000, 0.00000, -2.00000) -- (2.00000, 0.00000, -1.00000);
\draw[edge,back] (2.00000, -1.00000, 0.00000) -- (2.00000, 0.00000, -1.00000);
\draw[edge,back] (2.00000, -1.00000, 0.00000) -- (2.00000, 0.00000, 1.00000);
\draw[edge,back] (2.00000, 0.00000, -1.00000) -- (2.00000, 1.00000, 0.00000);
%%
%%
%% Drawing vertices in the back
%%
\node[vertex] at (1.00000, 0.00000, -2.00000)     {};
\node[vertex] at (2.00000, 0.00000, -1.00000)     {};
\node[vertex] at (2.00000, -1.00000, 0.00000)     {};
\node[vertex] at (0.00000, -3.00000, 0.00000)     {};
\node[vertex] at (0.00000, -1.00000, -2.00000)     {};
%%
%%
%% Drawing the facets
%%
\fill[facet] (2.00000, 1.00000, 0.00000) -- (0.00000, 3.00000, 0.00000) -- (0.00000, 1.00000, 2.00000) -- (1.00000, 0.00000, 2.00000) -- (2.00000, 0.00000, 1.00000) -- cycle {};
\fill[facet] (1.00000, 0.00000, 2.00000) -- (-2.00000, -3.00000, 2.00000) -- (-3.00000, -2.00000, 2.00000) -- (0.00000, 1.00000, 2.00000) -- cycle {};
\fill[facet] (0.00000, 3.00000, 0.00000) -- (-2.00000, 3.00000, -2.00000) -- (-3.00000, 2.00000, -2.00000) -- (-3.00000, -2.00000, 2.00000) -- (0.00000, 1.00000, 2.00000) -- cycle {};
%%
%%
%% Drawing edges in the front
%%
\draw[edge] (-3.00000, -2.00000, 2.00000) -- (-3.00000, 2.00000, -2.00000);
\draw[edge] (-3.00000, -2.00000, 2.00000) -- (-2.00000, -3.00000, 2.00000);
\draw[edge] (-3.00000, -2.00000, 2.00000) -- (0.00000, 1.00000, 2.00000);
\draw[edge] (-3.00000, 2.00000, -2.00000) -- (-2.00000, 3.00000, -2.00000);
\draw[edge] (-2.00000, -3.00000, 2.00000) -- (1.00000, 0.00000, 2.00000);
\draw[edge] (-2.00000, 3.00000, -2.00000) -- (0.00000, 3.00000, 0.00000);
\draw[edge] (0.00000, 1.00000, 2.00000) -- (0.00000, 3.00000, 0.00000);
\draw[edge] (0.00000, 1.00000, 2.00000) -- (1.00000, 0.00000, 2.00000);
\draw[edge] (0.00000, 3.00000, 0.00000) -- (2.00000, 1.00000, 0.00000);
\draw[edge] (1.00000, 0.00000, 2.00000) -- (2.00000, 0.00000, 1.00000);
\draw[edge] (2.00000, 0.00000, 1.00000) -- (2.00000, 1.00000, 0.00000);
%%
%%
%% Drawing the vertices in the front
%%
\node[vertex] at (-3.00000, -2.00000, 2.00000)     {};
\node[vertex] at (-3.00000, 2.00000, -2.00000)     {};
\node[vertex] at (-2.00000, -3.00000, 2.00000)     {};
\node[vertex] at (-2.00000, 3.00000, -2.00000)     {};
\node[vertex] at (0.00000, 1.00000, 2.00000)     {};
\node[vertex] at (0.00000, 3.00000, 0.00000)     {};
\node[vertex] at (1.00000, 0.00000, 2.00000)     {};
\node[vertex] at (2.00000, 0.00000, 1.00000)     {};
\node[vertex] at (2.00000, 1.00000, 0.00000)     {};
%%
%%
\end{tikzpicture}

==> tikz/perm3.tex <==
\begin{tikzpicture}%
	[x={(0.178656cm, 0.726606cm)},
	y={(-0.806737cm, 0.494173cm)},
	z={(0.563256cm, 0.477323cm)},
	scale=0.80000,
	back/.style={loosely dotted, thin},
	edge/.style={color=black, thick},
	facet/.style={fill=white,fill opacity=0.800000},
	vertex/.style={inner sep=1pt,circle,draw=black!25!black,fill=black!75!black,thick,anchor=base}]
%
%
%% Coordinate of the vertices:
%%
\coordinate (-2.00000, -1.00000, 0.00000) at (-2.00000, -1.00000, 0.00000);
\coordinate (-2.00000, 0.00000, -1.00000) at (-2.00000, 0.00000, -1.00000);
\coordinate (-2.00000, 0.00000, 1.00000) at (-2.00000, 0.00000, 1.00000);
\coordinate (-2.00000, 1.00000, 0.00000) at (-2.00000, 1.00000, 0.00000);
\coordinate (-1.00000, -2.00000, 0.00000) at (-1.00000, -2.00000, 0.00000);
\coordinate (-1.00000, 0.00000, -2.00000) at (-1.00000, 0.00000, -2.00000);
\coordinate (-1.00000, 0.00000, 2.00000) at (-1.00000, 0.00000, 2.00000);
\coordinate (-1.00000, 2.00000, 0.00000) at (-1.00000, 2.00000, 0.00000);
\coordinate (0.00000, -2.00000, -1.00000) at (0.00000, -2.00000, -1.00000);
\coordinate (0.00000, -2.00000, 1.00000) at (0.00000, -2.00000, 1.00000);
\coordinate (0.00000, -1.00000, -2.00000) at (0.00000, -1.00000, -2.00000);
\coordinate (0.00000, -1.00000, 2.00000) at (0.00000, -1.00000, 2.00000);
\coordinate (0.00000, 1.00000, -2.00000) at (0.00000, 1.00000, -2.00000);
\coordinate (0.00000, 1.00000, 2.00000) at (0.00000, 1.00000, 2.00000);
\coordinate (0.00000, 2.00000, -1.00000) at (0.00000, 2.00000, -1.00000);
\coordinate (0.00000, 2.00000, 1.00000) at (0.00000, 2.00000, 1.00000);
\coordinate (1.00000, -2.00000, 0.00000) at (1.00000, -2.00000, 0.00000);
\coordinate (1.00000, 0.00000, -2.00000) at (1.00000, 0.00000, -2.00000);
\coordinate (1.00000, 0.00000, 2.00000) at (1.00000, 0.00000, 2.00000);
\coordinate (1.00000, 2.00000, 0.00000) at (1.00000, 2.00000, 0.00000);
\coordinate (2.00000, -1.00000, 0.00000) at (2.00000, -1.00000, 0.00000);
\coordinate (2.00000, 0.00000, -1.00000) at (2.00000, 0.00000, -1.00000);
\coordinate (2.00000, 0.00000, 1.00000) at (2.00000, 0.00000, 1.00000);
\coordinate (2.00000, 1.00000, 0.00000) at (2.00000, 1.00000, 0.00000);
%%
%%
%% Drawing edges in the back
%%
\draw[edge,back] (-1.00000, -2.00000, 0.00000) -- (0.00000, -2.00000, -1.00000);
\draw[edge,back] (-1.00000, 0.00000, -2.00000) -- (0.00000, -1.00000, -2.00000);
\draw[edge,back] (0.00000, -2.00000, -1.00000) -- (0.00000, -1.00000, -2.00000);
\draw[edge,back] (0.00000, -2.00000, -1.00000) -- (1.00000, -2.00000, 0.00000);
\draw[edge,back] (0.00000, -2.00000, 1.00000) -- (1.00000, -2.00000, 0.00000);
\draw[edge,back] (0.00000, -1.00000, -2.00000) -- (1.00000, 0.00000, -2.00000);
\draw[edge,back] (0.00000, 1.00000, -2.00000) -- (1.00000, 0.00000, -2.00000);
\draw[edge,back] (1.00000, -2.00000, 0.00000) -- (2.00000, -1.00000, 0.00000);
\draw[edge,back] (1.00000, 0.00000, -2.00000) -- (2.00000, 0.00000, -1.00000);
\draw[edge,back] (2.00000, -1.00000, 0.00000) -- (2.00000, 0.00000, -1.00000);
\draw[edge,back] (2.00000, -1.00000, 0.00000) -- (2.00000, 0.00000, 1.00000);
\draw[edge,back] (2.00000, 0.00000, -1.00000) -- (2.00000, 1.00000, 0.00000);
%%
%%
%% Drawing vertices in the back
%%
\node[vertex] at (1.00000, 0.00000, -2.00000)     {};
\node[vertex] at (2.00000, 0.00000, -1.00000)     {};
\node[vertex] at (2.00000, -1.00000, 0.00000)     {};
\node[vertex] at (0.00000, -2.00000, -1.00000)     {};
\node[vertex] at (0.00000, -1.00000, -2.00000)     {};
\node[vertex] at (1.00000, -2.00000, 0.00000)     {};
%%
%%
%% Drawing the facets
%%
\fill[facet] (2.00000, 1.00000, 0.00000) -- (1.00000, 2.00000, 0.00000) -- (0.00000, 2.00000, 1.00000) -- (0.00000, 1.00000, 2.00000) -- (1.00000, 0.00000, 2.00000) -- (2.00000, 0.00000, 1.00000) -- cycle {};
\fill[facet] (-2.00000, 1.00000, 0.00000) -- (-2.00000, 0.00000, -1.00000) -- (-2.00000, -1.00000, 0.00000) -- (-2.00000, 0.00000, 1.00000) -- cycle {};
\fill[facet] (1.00000, 0.00000, 2.00000) -- (0.00000, -1.00000, 2.00000) -- (-1.00000, 0.00000, 2.00000) -- (0.00000, 1.00000, 2.00000) -- cycle {};
\fill[facet] (0.00000, 2.00000, -1.00000) -- (-1.00000, 2.00000, 0.00000) -- (-2.00000, 1.00000, 0.00000) -- (-2.00000, 0.00000, -1.00000) -- (-1.00000, 0.00000, -2.00000) -- (0.00000, 1.00000, -2.00000) -- cycle {};
\fill[facet] (0.00000, 2.00000, 1.00000) -- (-1.00000, 2.00000, 0.00000) -- (-2.00000, 1.00000, 0.00000) -- (-2.00000, 0.00000, 1.00000) -- (-1.00000, 0.00000, 2.00000) -- (0.00000, 1.00000, 2.00000) -- cycle {};
\fill[facet] (1.00000, 2.00000, 0.00000) -- (0.00000, 2.00000, -1.00000) -- (-1.00000, 2.00000, 0.00000) -- (0.00000, 2.00000, 1.00000) -- cycle {};
\fill[facet] (0.00000, -1.00000, 2.00000) -- (-1.00000, 0.00000, 2.00000) -- (-2.00000, 0.00000, 1.00000) -- (-2.00000, -1.00000, 0.00000) -- (-1.00000, -2.00000, 0.00000) -- (0.00000, -2.00000, 1.00000) -- cycle {};
%%
%%
%% Drawing edges in the front
%%
\draw[edge] (-2.00000, -1.00000, 0.00000) -- (-2.00000, 0.00000, -1.00000);
\draw[edge] (-2.00000, -1.00000, 0.00000) -- (-2.00000, 0.00000, 1.00000);
\draw[edge] (-2.00000, -1.00000, 0.00000) -- (-1.00000, -2.00000, 0.00000);
\draw[edge] (-2.00000, 0.00000, -1.00000) -- (-2.00000, 1.00000, 0.00000);
\draw[edge] (-2.00000, 0.00000, -1.00000) -- (-1.00000, 0.00000, -2.00000);
\draw[edge] (-2.00000, 0.00000, 1.00000) -- (-2.00000, 1.00000, 0.00000);
\draw[edge] (-2.00000, 0.00000, 1.00000) -- (-1.00000, 0.00000, 2.00000);
\draw[edge] (-2.00000, 1.00000, 0.00000) -- (-1.00000, 2.00000, 0.00000);
\draw[edge] (-1.00000, -2.00000, 0.00000) -- (0.00000, -2.00000, 1.00000);
\draw[edge] (-1.00000, 0.00000, -2.00000) -- (0.00000, 1.00000, -2.00000);
\draw[edge] (-1.00000, 0.00000, 2.00000) -- (0.00000, -1.00000, 2.00000);
\draw[edge] (-1.00000, 0.00000, 2.00000) -- (0.00000, 1.00000, 2.00000);
\draw[edge] (-1.00000, 2.00000, 0.00000) -- (0.00000, 2.00000, -1.00000);
\draw[edge] (-1.00000, 2.00000, 0.00000) -- (0.00000, 2.00000, 1.00000);
\draw[edge] (0.00000, -2.00000, 1.00000) -- (0.00000, -1.00000, 2.00000);
\draw[edge] (0.00000, -1.00000, 2.00000) -- (1.00000, 0.00000, 2.00000);
\draw[edge] (0.00000, 1.00000, -2.00000) -- (0.00000, 2.00000, -1.00000);
\draw[edge] (0.00000, 1.00000, 2.00000) -- (0.00000, 2.00000, 1.00000);
\draw[edge] (0.00000, 1.00000, 2.00000) -- (1.00000, 0.00000, 2.00000);
\draw[edge] (0.00000, 2.00000, -1.00000) -- (1.00000, 2.00000, 0.00000);
\draw[edge] (0.00000, 2.00000, 1.00000) -- (1.00000, 2.00000, 0.00000);
\draw[edge] (1.00000, 0.00000, 2.00000) -- (2.00000, 0.00000, 1.00000);
\draw[edge] (1.00000, 2.00000, 0.00000) -- (2.00000, 1.00000, 0.00000);
\draw[edge] (2.00000, 0.00000, 1.00000) -- (2.00000, 1.00000, 0.00000);
%%
%%
%% Drawing the vertices in the front
%%
\node[vertex] at (-2.00000, -1.00000, 0.00000)     {};
\node[vertex] at (-2.00000, 0.00000, -1.00000)     {};
\node[vertex] at (-2.00000, 0.00000, 1.00000)     {};
\node[vertex] at (-2.00000, 1.00000, 0.00000)     {};
\node[vertex] at (-1.00000, -2.00000, 0.00000)     {};
\node[vertex] at (-1.00000, 0.00000, -2.00000)     {};
\node[vertex] at (-1.00000, 0.00000, 2.00000)     {};
\node[vertex] at (-1.00000, 2.00000, 0.00000)     {};
\node[vertex] at (0.00000, -2.00000, 1.00000)     {};
\node[vertex] at (0.00000, -1.00000, 2.00000)     {};
\node[vertex] at (0.00000, 1.00000, -2.00000)     {};
\node[vertex] at (0.00000, 1.00000, 2.00000)     {};
\node[vertex] at (0.00000, 2.00000, -1.00000)     {};
\node[vertex] at (0.00000, 2.00000, 1.00000)     {};
\node[vertex] at (1.00000, 0.00000, 2.00000)     {};
\node[vertex] at (1.00000, 2.00000, 0.00000)     {};
\node[vertex] at (2.00000, 0.00000, 1.00000)     {};
\node[vertex] at (2.00000, 1.00000, 0.00000)     {};
%%
%%
\end{tikzpicture}
